Cosine-Pruned Medial Axis: A new method for isometric equivariant and noise-free medial axis extraction

We present the CPMA, a new method for medial axis pruning with noise robustness and equivariance to isometric transformations. Our method leverages the discrete cosine transform to create smooth versions of a shape $\Omega$. We use the smooth shapes to compute a score function $\scorefunction$ that filters out spurious branches from the medial axis. We extensively compare the CPMA with state-of-the-art pruning methods and highlight our method's noise robustness and isometric equivariance. We found that our pruning approach achieves competitive results and yields stable medial axes even in scenarios with significant contour perturbations.

==> sections/09_other.tex <==
%these different approaches to shape analysis but also unveil the latest efforts in the scientific community. A comprehensive review of the main shape analysis approaches will be offered along with its applications and challenges.

\section{Overview of the Stated Problem}

In this dissertation, we study the problem of describing the shape of an object in 2D and 3D with a set of features invariant to isometric transformations, particularly rotations. We focus our approach on the well-known Medial Axis Transform (MAT) and its topological properties. A set of experiments conducted on popular datasets was performed to highlight how our descriptor behaves compared with state-of-the-art approaches. 

We aim to study two problems. The first problem: how to find a shape representation of a segmented object that exhibits rotation, translation,  and reflection invariance. The second problem: how to build a machine learning pipeline that uses the isometric invariance of the shape representation to do both classification and retrieval. Our proposed solution demonstrates competitive results compared to state-of-the-art approaches.

We base our descriptor on the MAT, sometimes called a topological skeleton. Accepted and well-studied properties of the medial axis include~\citep{Manzanera1999}:

\begin{description}
    \item[Homotopy] skeletons must preserve the topology of the original shapes/images.
    \item[One-pixel thickness] skeletons should be made of one-pixel thick lines.
    \item [Mediality] they should be positioned in the middle of shapes (with all skeleton points having the same distance from two closest points on object boundary).
    \item [Rotation invariance] in discrete spaces, this can only be satisfied for rotation angles, which are multiples of $\frac{\pi}{2}$ but should be approximately satisfied for other angles.
    \item [Noise immunity] skeletons should be insensitive to shape-boundary noise.
    \item [Reconstruction] one should be capable of reconstructing the original object from the skeleton.
\end{description}

These properties make the MAT a suitable input to create a shape descriptor; however, several problems arise because not all skeletonization methods satisfy all of these properties at the same time. In general, skeletons based on thinning approaches preserve topology but are noise sensitive and do not allow for proper reconstruction of the original shape. These skeletons are also not invariant to rotations. 

Voronoi skeletons also preserve topology and are rotation invariant, but do not include information about the thickness of the object, which makes reconstruction impossible. The Voronoi skeleton is an approximation of the real skeleton. The denser the sampling of the boundary, the better the approximation; however, a denser sampling makes the Voronoi diagram more computationally expensive.

In contrast, distance transform methods allow the reconstruction of the original object by providing the distance from every pixel in the skeleton to the boundary. Moreover, they exhibit an acceptable degree of the MAT properties listed above, but noise sensitivity remains an issue. Given this information, we selected distance transform medial axis methods as our skeletonization strategy and focused on creating a new noise-free approach to solve the contour noise problem.

% from SAHA
Most skeletonization methods produce a skeleton that contains many more branches than desired, which can occur for several reasons. The most common reason is border noise, where every little protrusion gives rise to a skeletal branch. Unwanted parts of the skeleton are called spurious branches. Many skeletonization methods deal with spurious branches through the process of pruning, where the spurious branches are removed. In those cases, what defines a spurious part must be determined either while computing the skeleton or as a post-processing step.

To effectively classify an object, or perform any other task with features based on the object shape, the descriptor needs to be a normalized, compact form: a map $\Phi$ that take every shape $\Omega$ to the same vector space $\mathrm{R}^{n}$. This is not possible with skeletonization methods because the skeletons of different objects have different numbers of branches and different numbers of points, even when they belong to the same category. Consequently, we developed a strategy to extract features from the skeleton through the map $\Phi$, which we used as an input to a machine learning approach.

In this study, we sought to design an isometric invariant shape descriptor through robust skeletonization enforced by a feature extraction pipeline that exploits such invariance through a machine learning methodology. We conducted a set of classification and retrieval experiments over well-known benchmarks to validate our proposed method.

\section{Methodology Design}
\label{sec:methodology_design}

\subsection{Robust Skeletonization}
\label{subsec:robust_skeletonization}

Spurious branches in the MAT are generally associated with noise in the contour. Even small perturbation can cause a new branch to appear. Spurious branches create an erroneous underlying structure of the object (Figure \ref{fig:example_spurious_branch}). We refer to any method that outputs a consistent skeleton in the presence of several degrees of noise: ``robust skeletonization''. 

One strategy for removal of spurious branches consists of directly smoothing the shape~\citep{Rumpf2002,Mokhtarian1992789}, which results in a $\mathbf{MAT}$ with less noise. The filtered skeleton of the unfiltered shape is later defined as the unfiltered skeleton of the filtered shape. The main drawback of this approach is that, in most cases, the resulting medial axis is not a good approximation of the real medial axis (RMA). Additionally, the smoothing procedure can potentially change the topology of the shape resulting in a different skeleton.  Miklos~\cite{Miklos:2010:DSA:1778765.1778838} introduced a slightly different approach with the Scaled Axis Transform (SAT). The SAT involves applying a scale transformation to the distance map and computing the unfiltered medial axis of the resulting reconstructed shape. In~\citep{Postolski2014}, the authors highlighted the fact that the Scale Axis Transform is not necessarily a subset of the original shape, and went beyond Miklos' work to propose a solution that guarantees a better approximation of the RMA.

%TODO: put the second row of images with spurious branches in 3D
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.39\linewidth}
        \includegraphics[width=\linewidth]{images/contour_protusion.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.39\linewidth}
        \includegraphics[width=\linewidth]{images/spourious_branches.png}
    \end{subfigure}
    
    \caption[Spurious branch in medial axis.]{Spurious branch in medial axis. A new whole branch appear (right), even when a small perturbation of the contour (left).}
     \label{fig:example_spurious_branch}
\end{figure}

One of the most popular solutions to spurious branches~\citep{Couprie2007} considered the angle formed by a point $p \in \Omega$, and its two closest boundary points $\Pi_{\Omega}(x)$, called the distance transform of $p$. This solution removes skeleton points for which this angle is lower than a fixed threshold. This criterion allows different scales within a shape but generally leads to an unconnected medial axis. Some modifications to his approach have been proposed. In \citep{Hesselink2008}, the authors introduced the Gamma $\gamma$-Integer Medial Axis (GIMA), where a point belongs to the skeleton if the distance between its two closest boundary points is at least equal to $\gamma$.

All the work mentioned above is based on the distance transform $\mathcal{D}_{\Omega}(x)$. The distance transform acts as a generator function for the medial axis, such that points $p \in \mathbf{MAT}$ if and only if they satisfy some constraint involving their distance to the boundary. However, by itself, the distance transform poses some problems because it usually contains discontinuities. See figure \ref{fig:distance_transform_discontinuity}. As a result, some studies focus on extracting alternative generator functions. An example is  \citep{Gorelick2006}, where they proposed to estimating $\mathcal{D}_{\Omega}(x)$ as the solutions of the Poisson equation

\begin{equation}
    \Delta u(x) = -1.
\end{equation}

Later, \citep{Aubert2014} formalized the concept of the Poisson Skeleton and provided the details of a skeletonization algorithm based on this principle. Poisson skeletons rely on a solid mathematical formulation. Among other concepts, they use the local minimums and maximums of the curvature of $\delta \Omega$. However, when such methodology is applied in a discrete environment, many spurious branches appear due to the need to define the length of a kernel size to estimate these local extreme points. 

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/distance_transform_discontinuity.png}
    
    \caption[Distance transform discontinuities.]{Distance transform discontinuities. The image in the left shows the Euclidean distance of each point to the contour of the object. Notice how some discontinuities appear near the areas where the level sets change curvature. The image on the right shows an at least twice differentiable approximation of $u$ using \cite{Gorelick2006} approach.}
    \label{fig:distance_transform_discontinuity}
\end{figure}

In contrast to the studies mentioned above, we propose a method to prune the medial axis and free it from as many spurious branches as possible without compromising the reconstruction property. Our method must preserve the topology and connectivity of the original object while maintaining its equivariance to isometric transformations.

Let $\Omega$ be an n-dimensional closed shape with a boundary $\delta \Omega$. We propose a new pruning approach to robust skeletonization by filtering the $\mathbf{MAT}$ of $\Omega$ with a score function $\scorefunction(X): \mathbb{N}^{2} \mapsto \mathbb{R}^{+}$. The function $\scorefunction$ acts as an indication of the relevance of point $X$ in the \textbf{real} skeleton of $\Omega$. We define $\scorefunction$ as the average of a set of estimation of the $\mathbf{MAT}$ over smoothed versions $\hat{\Omega}$ of the original object. Intuitively, $\scorefunction$ acts as a sort of probability of how likely it is for a point $X$ to belong to the real skeleton of $\Omega$. The real skeleton branches will regularly appear in the skeletons resulting in high values of the score function. In contrast, spurious branches will only appear occasionally, resulting in low values. 

%of a set $\mathbf{S}(\Omega) = \left \{ S_{i} | i=1,...,m \right \} $ of naive estimations of the medial axis of a shape $\Omega$ under different levels of a smoothed contour. 

%In this context, we refer to a naive estimation to any distance transform based approach to calculate the MAT that still is prone to produce spurious branches. 

% Source for the equations: https://unix4lyfe.org/dct/

To create the set of medial axis from the smoothed boundary, we used the Discrete Cosine Transform (DCT). The DCT in two dimensions has the form:

\begin{displaymath}
    \arraycolsep=1.4pt\def\arraystretch{1.5}
    \begin{array}{l}
         C_{u} = \left \{ 
                    \begin{array}{cc}
                        \frac{1}{\sqrt{2}} & \textrm{if } u = 0 \\
                        1 & \textrm{otherwise} \\
                    \end{array} \right. \\
         C_{v} = (\textrm{Similar to above})  \\
    \end{array}
\end{displaymath}
\smallskip
\begin{displaymath}
    \mathfrak{F}(u, v) = \frac{1}{4}C_{u}C_{v}\sum_{x=0}^{N-1}\sum_{y=0}^{M-1} \mathcal{I}(x, y)cos \left( u\pi \frac{2x+1}{2N} \right) cos \left( v\pi \frac{2y+1}{2M}\right)
\end{displaymath}
                
Where $(u,v)$ are the frequency coordinates in the frequency domain. 

The DCT is closely related to the discrete Fourier transform of real valued-functions. The DCT, however, has better energy compaction properties, with just a few of the transform coefficients representing the majority of the energy in the sequence. Multidimensional variants of the various DCT types follow straightforwardly from the one-dimensional definitions: they are simply a separable product (equivalently, a composition) of DCTs along each dimension.

Mathematically, the DCT is perfectly reversible and does not lose any image information. To rebuild an image in the spatial domain from the frequencies obtained above, we use the IDCT:

\begin{equation}
    \mathcal{I}(x, y) = \frac{1}{4}\sum_{u=0}^{N-1}\sum_{v=0}^{N-1} C_{u}C_{v}\mathfrak{F}(u, v) cos \left( u\pi \frac{2x+1}{2N} \right) cos \left( v\pi \frac{2y+1}{2N}\right).
    \label{eq:rec_IDCT}
\end{equation}

For the n-dimensional DCT we will use the notation $\mathcal{I}(X)$, with $X \in \mathbb{R}^{n}$, instead of $\mathcal{I}(x, y)$.

Additionally, we denote $\hat{\mathcal{I}}^{(M)}$ as the reconstructed version of $\mathcal{I}$ using only the first $M$ frequencies of the DCT in equation \ref{eq:rec_IDCT}, with $M < N$. Now, we are ready to define our pruning strategy based on these concepts.

We define the \textbf{Cosine-Pruned Medial Axis} (CPMA) as a pruned version of the $\mathbf{MAT}$ of a shape $\Omega$. The $\mathbf{CPMA}(\Omega)$ consist of all the pairs $(X, r) \in \mathbf{MAT}(\Omega)$ such that the score function evaluated on $X$ is greater than a threshold $\tau$. e.g. $\scorefunction(X) > \tau$. The score function is defined as

\begin{equation}
    \scorefunction(X) = \frac{1}{M}\sum_{i=1}^{M} [\mathbf{MAT}( \hat{\mathcal{I}}^{(i)})](X).
    \label{eq:score_function}
\end{equation}

The value of $\tau$ was determined empirically; however, we conducted an additional set of experiments to show how sensitive the CPMA is to different values of the threshold.

Although the CPMA results in a noise-free medial axis, its definition also allows disconnected skeletons. There is no restriction in its formulation to force individual elements of the CPMA to create a connected skeleton. We solved this issue by finding individual disconnected pieces of the CPMA and representing each piece as a graph. Later, we connect them using a geodesic distance $g(n_{i}, n_{j})$ inside $\Omega$, where $n_{i}$ and $n_{j}$ where are nodes of two distinct pieces. However, the geodesic distance can lead to a connection between nodes that do not follow the medial axis (See figure \ref{fig:cpma_connectivity}). To address this, we instead compute the minimum energy distance between $n_{1}$ and $n_{2}$ using the inverse score function as energy field, $E_{\Omega} = 1 - \scorefunction$. Because $\scorefunction$ is bounded on the interval $[0, 1]$, we guaranty that $E_{\Omega}(X)$ will have higher values as $X$ is close to $\delta \Omega$, and lower values when $X$ is close to the centerline of the object, hence forcing the paths to be close to the MAT. We call the result of connecting all the pieces the Connected CPMA.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/graph_connectivity.png}
    \caption[Path connectivity between CPMA segments]{Path connectivity between CPMA segments. When using the euclidean distance (left), two nodes could connect through a path that is not entirely contained inside the object $\Omega$. The minimum geodesic distance (center) guarantees that the path will be inside the object, but does not follow the centerline. The minimum energy distance with $\scorefunction$ as the energy field is the best alternatives and forces the path to follow the medial axis. }
    \label{fig:cpma_connectivity}
\end{figure}

In the next chapter, we will offer additional details about our method for robust skeletonization. We will present the implementation details of the concepts described above, as well as the algorithms and experiment results to support our claims.

\subsection{Design of a Skeleton-Based Shape Descriptor}

In this subsection, we describe the feature extraction mechanism to map the skeleton-based features discussed above to a set features $\phi$. We also describe the machine learning pipeline that takes $\phi$ as input and processes it to do both shape classification and retrieval. We will also show how the selected machine learning architecture preserves the invariant properties of the skeleton of the shape.

%\textbf{P}Other approaches for shape classification. *taken from Carlos's paper and state of the art. First, explain classic methods.


To extract a set of features from the skeleton representation of $\Omega$ through the use of the \textbf{Chordiogram} defined by \cite{Toshev2011}. The chordiogram is a rotation and translation invariant shape descriptor capturing global geometric relationships between elements of the object boundary. To define the chordiogram, consider a pair of boundary edges $p$ and $q$ from $\delta \Omega$. We will call such a pair $(p,q)$ a chord. One can define various features that describe the geometry of the chord, which we will denote by $f_{pq} \in \mathbb{R}^{d}$, as we will see in chapter \ref{ch:classificaton_method}. The chordiogram is defined as the k-dimensional histogram of $f_{pq}$ over all the chords. By carefully defining $f_{pq}$, and because isometric transformations are equally applied to all points in the object, the chordiogram is able to capture the invariant properties of $\Omega$. e.g., if we set $f^{0}_{pq}$ as the euclidean distance between $p$ and $q$, and set $R$ as a rotation around the origin of coordinates; then we have that

\begin{equation}
     ||Rp - Rq|| = ||R(p-q)|| = \sqrt{(p-q)^{T}R^{T} R (p-q)} = (p-q)^{T}(p-q) = ||p-q||,
     \label{eq:euc_dist_invariance}
\end{equation}

Because $R$ is a unitary matrix. Figure \ref{fig:chord_formation} shows how the chords are formed on a 2D shape.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/chord_computation.png}
    \caption[Computation of individual chord in the chordiogram]{Computation of individual chord in the chordiogram. Images a), b) c) shows examples of different chords from point pairs $(p_{1}, q_{1})$ and $(p_{2}, q_{2})$, an some of the properties that can extracted from them.}
    \label{fig:chord_formation}
\end{figure}

Two problems quickly arise from the definition of the chordiogram. First, the chordiogram depends on the relationships of pairs of points in the boundary, and then it needs a dense sampling to cover all the geometry of the object properly. Moreover, a dense sampling, such as $n$ points sampled from $\delta \Omega$, leads to a significantly large number of chords, $\#chords = n(n - 1)$. This number quickly becomes intractable even for up-to-date computational resources, especially in the 3D case. With a small $n$, the risk is not to have enough representative points from the contour to capture its geometric properties. 

The second problem is the noise of the boundary. As in the case of the medial axis, boundary noise can cause variation of the final computation of the chordiogram. In this case, the noise is represented as jittering on the ends of the chords, slightly changing their features. Although a good machine learning approach acting on a set of features should be robust to these types of artifacts in the data, this effect should be minimized.

%--------------
To deal with sampling and boundary jittering problems, we will use results from subsection \ref{subsec:robust_skeletonization}. After computing the CPMA of $\Omega$, we use it to extract chords from the joints of the skeleton, not from the boundary points. This is done to 1) reduce the total number of chords representing the object. Notice that the chords computed over the skeleton maintain the isometric invariances discussed in subsection \ref{subsec:robust_skeletonization}. 

%\textbf{P}The chordiogram applied to skeletons. State the sampling is better because we can use all skeleton chords. The noise-free skeleton, reduces uncertainty to noise contour. But with a cost, induces ambiguity. 
%--------------

Convolutional neural networks have shown that jointly optimizing feature extraction and classification pipelines can significantly improve object recognition~\citep{Lecun1998,NIPS2012_4824}. Applying CNNs for shape analysis, however, is not as straightforward as one might think. CNN learning strategy is based on learning a set of features that are applied to the input as convolution filters. These mechanisms benefit from uniform grid structures of images in 2D, where convolutions can be computed via sliding windows; however, shape information is stored in different ways. In 2D, the segmented mask of a shape is a binary image where there is not enough photometric variation in the image for the filters to learn useful features. Therefore,  more preferable formats are used to obtain the shape information, e.g., a sample point cloud from the contour of the object. This strategy is especially useful in 3D, where information is typically represented as a point cloud or 3D triangular mesh.

For this reason, we chose to use PointNets~\citep{Qi2017PointNetDL,qi2017pointnetplusplus} as the machine learning model for our experiments. PointNets are deep learning architectures that directly consume raw point clouds without converting them to other formats. They have been applied to single object classification and semantic segmentation. Additionally, one of the key design aspects of PointNets is their invariance to permutations of the input points, which facilitates the learning process in datasets of objects coming from different sensors, resolutions of scales.

We combined our skeleton-based approach with the most recent and widely used architecture (PointNet++ arch~\citep{qi2017pointnetplusplus}). We did this by setting the list of $N$ chords computed from the skeleton of $\Omega$ as input for the neural network.  The model determined by 

\begin{equation}
    \hat{Y} = \mathcal{L}_{\theta}(X) 
\end{equation}

Where $\theta$ is the parameter vector to train, and $X \in \mathbb{R}^{N \times K}$ is a list of $N$ chords each one with $K$ features. The network was trained using the classification cross-entropy as the loss function. After training, the learned latent space, the layer before the fully-connected part of the network, was used as a feature vector for retrieval. %Figure \ref{fig:chord_plus_pointnet_arch} described the full architecture.

In the next section, we will describe the experimental setup that was used to evaluate our proposed method. 

\section{Experimental setup}

In this section, we explain in detail the experimental framework we used to evaluate the proposed descriptor. As we described in section \ref{sec:methodology_design}, our approach to solve the stated problem has two main components: 1) a skeleton computation method that is robust to spurious branches; especially those coming from the noise in the contour of the object, and 2) the design of shape classification architecture based on features extracted from the topological skeleton. Thus, we designed a series of experiments to test each component of our solution in comparison to the state-of-the-art. We performed our experiments on available datasets of 2D silhouettes and 3D models in mesh format. Additionally, we employed well-known metrics to assess the main properties of our solution.

\subsection{Datasets}

We chose five extensively used datasets of 2D and 3D data to evaluate our methodology on skeletonization robustness, classification, and retrieval accuracy.  These datasets are part of the accepted benchmarks in literature, which enabled us to compare our results to previous work.

\paragraph{Kimia216} In our comparative study, we used the Kimia-216 shape dataset~\citep{Sebastian2004} to test skeletonization robustness. It consists of 18 classes of different shapes with 12 samples in each class. The images in the dataset represent a collection of slightly different views of a set of shapes with different topologies. Contour noise and random rotations are also present in some of the images in the dataset. Kimia216 has been largely used to test a wide range of skeletonization algorithms. Because of this, and the large variety of shapes, we assumed that this benchmark ensured a fair comparison with the state-of-the-art regarding skeletonization methods. Figure \ref{fig:example_kimia_216} shows two samples from each class.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/kimia_example.jpg}
    \caption[Examples from Kimia 216 dataset]{Kimia 216 dataset: Two samples shapes from each class.}
    \label{fig:example_kimia_216}
\end{figure}

\paragraph{Animal Dataset} We used the Animal2000~\citep{Bai2009} dataset to evaluate the performance of our skeleton representation with respect to articulations of the object; as a way to show the benefits of our proposed skeletonization method when facing non-rigid transformations. The Animal2000 database has 2000 images of 20 categories; each category consists of 100 images (Figure \ref{fig:example_animal_dataset}). Because silhouettes in Animal2000 were obtained from real images, each class is characterized by a large intra-class variation in shape.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/animal_dataset.png}
    \caption[Sample shapes from Animal2000 database.]{Sample shapes from Animal2000 database.}
    \label{fig:example_animal_dataset}
\end{figure}

\paragraph{MPEG7} We also experimented on the MPEG-7 CE-Shape 1 part B dataset~\citep{Latecki2000}. This dataset is commonly used for the evaluation of shape-based classification and retrieval. It consists of 1400 binary object masks representing 70 different classes, each class including 20 examples. The metric employed to evaluate results on this dataset is the Bull's eye score: each shape is matched to all shapes, and the percentage of the 20 possible correct matches among the top 40 matches is recorded. The Bull's score is the average percentage of overall shapes. See Figure \ref{fig:example_mpeg7_dataset}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/Samples-from-MPEG7-Set-B-dataset_W640.jpg}
    \caption[Examples from MPEG7 dataset]{Examples from MPEG7 dataset: One sample from each category is shown.}
    \label{fig:example_mpeg7_dataset}
\end{figure}

\paragraph{ModelNet} The main 3D dataset we used in this study is the well-known Princeton ModelNet-40 large-scale 3D CAD model dataset~\citep{7298801}. ModelNet-40 comprises 12.311 CAD models split into 40 categories. Additionally, the dataset splits into training and testing subsets containing 9843 and 2468 models, respectively. The models have been manually cleaned and normalized to fit into a unit sphere. ModelNet40 is often used as the benchmark for 3D shape recognition, shape classification and shape retrieval tasks~\citep{Qi2017PointNetDL,Su2015MVCNN}; for this reason, it is suitable to evaluate the accuracy of the classification methodology developed in this dissertation. A rendered example from some categories can be referenced in Figure \ref{fig:example_modelnet_40}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.8\linewidth]{images/modelnet_example.png}
    \caption[Examples from ModelNet-40 dataset]{ModelNet-40 dataset: Rendered images from some of the 40 classes are shown in arbitrary poses.}
    \label{fig:example_modelnet_40}
\end{figure}

\paragraph{University of Groningen Skeletonization Benchmark} This set is commonly found in the literature to evaluate skeletonization methods in 3D~\citep{Sobiecki2014,Sobiecki2013,Chaussard2011}. It includes natural as well as synthetic shapes taken from other popular datasets. It includs shapes with and without (multiple) holes, of varying thickness, and with smooth and noisy boundaries. Shapes are provided in PLY triangle mesh format\footnote{http://www.cs.rug.nl/svcg/Shapes/SkelBenchmark}. All meshes have been cleaned to ensure a consistent orientation, closeness, no duplicate or T vertices, and no degenerate faces. Each file describes a single connected shape. Mesh resolutions range between a few thousand vertices and over a million vertices. See Figure \ref{fig:examples_groningen_benchmark}.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=\linewidth]{images/gronigen.png}
    \caption[Groningen Skeletonization Benchmark]{Groningen Skeletonization Benchmark: Examples of some of the in the dataset.}
    \label{fig:examples_groningen_benchmark}
\end{figure}

\subsection{Skeletonization Sensitivity Analysis}

In order to compare the robustness of any skeletonization method, we adopted an evaluation strategy similar to the one presented in \citep{Chaussard2011}. Consequently, we measured the similarity between the medial axis of a shape $\Omega$ and the one of shape $\Omega^{\prime}$ derived from a ``perturbation'' of $\Omega$. We were interested in evaluating how well our methodology would respond to the induced noise of the contour/surface of the object, which is a well-understood cause of spurious branches. We were also interested in assessing how stable the medial axis is in the presence of rotations to test for invariance to this isometric transformation.

As for similarity metrics, we employed the Hausdorff distance ($d_{H}$), and Dubuisson-Jain dissimilarity ($d_{D}$). The Dubuisson-Jain similarity is essentially a normalization of the Hausdorff distance using the size of the set involved in the computation~\citep{Dubuisson2002}, to help to overcome $d_{H}$ sensitivity to outliers. The Dubuisson-Jain similarity is defined as

\begin{equation}
d_{D}(X, Y) = max \left \{ D(X|Y), D(Y|X) \right \},
\label{eq:dubuison_jain_disimilarity}
\end{equation}
with 
\begin{equation}
D(X|Y) = \frac{1}{|X|}\sum_{x \in X} \min _{y \in Y} \left \{ d(x, y) \right\}.
\end{equation}

To evaluate the noise sensitivity, we must first choose a strategy to induce noise to the boundary of the object. We used a stochastic approach where a point $p$ and its neighbors $N(p)$ are deformed by a vector $v$ in the direction orthogonal to the boundary, and a deformation magnitude normally distributed, $|v| \sim \mathcal{N}(\mu=p, \sigma=1)$.  

This noise model is recurrently applied $n$ time to every shape in our datasets. We denote as $\mathbf{MAT}_{i}(\Omega)$ the medial axis of a shape $\Omega$ after applying the noise model $i$ times. To determine how invariant a particular skeletonization method is to boundary noise, we compared the original medial axis $\mathbf{MAT}(\Omega)$ with the noisy version of it $\mathbf{MAT}_{i}(\Omega)$ using both similarity metrics. We use similarity over all the elements in the dataset as the measurement of the invariance of the skeletonization method.

Regarding rotation sensitivity, the medial axis is ideally a rotation-invariant shape descriptor so that $\textrm{MA}(R(\Omega)) = R(\textrm{MA}(\Omega))$. See equation \ref{eq:invariance}. Due to sampling factors, this relationship is merely an approximation. However, we can measure how ``invariant'' a medial axis is by comparing $\mathbf{MAT}(R(\Omega))$ with $R(\mathbf{MAT}(\Omega))$ for different objects, and different definitions of the medial axis. The more similar they are, on average, the more invariant the skeletonization method is at computing the medial axis.

Rotations range from $0$ degrees to $90$ degrees counterclockwise around the origin for 2D objects in our experiments. In 3D, we used a combination of azimuthal ($\theta=[0, \frac{\pi}{2}]$) and elevation ($\phi=[0, \frac{\pi}{2}]$) rotations around the origin, so that the final rotation matrix is:
\begin{equation}
R=R_{az}(\theta)R_{el}(\phi)
\label{eq:rotation_matrix_rotation_sensitivity}
\end{equation}

Both the noise sensitivity and the rotation sensitivity tests were conducted on Kimia’s and Animal2000 datasets in 2D. For the 3D case, we usesd the Groningen Skeletonization Benchmark.

%A rotation can be described with a rotation matrix $R$. In the 2D case is possible to parametrize $R$ with a angle $\theta$ describing a contour-clock-wise rotation around the origin, $R_{\theta}$. In $\mathbb{R}^{3}$ 


%We first introduce some notions that will help us to ensure a fair comparison between methods, for which the filtering parameter does not have the same meaning.

%To introduce noise to the boundary of an object we propose deforming it using a process derived from the Eden’s (accretion) process [20]. The Eden’s process is an iterative random cellular automaton which, in its simplest form, attributes an equal probability to all the outer border points to be set to 1 at each step. That is, at each step, a neighbour of the object is chosen randomly and added to the shape. In spite of its simplicity, the Eden’s process exhibits good asymptotic isotropy [26]. In our process, we required accretion steps to deal only with simple points. This way at each step, the object’s homotopy type remains unchanged.

\subsection{Shape Classification and Retrieval}

One of the goals of this dissertation is to tackle the problem of invariance to isometric transformation. We, therefore, focused our experiments on problems that benefit from such invariance, namely, shape classification and retrieval in arbitrary orientations. We conducted shape classification and shape retrieval experiments on the MPEG7 and ModelNet-40 datasets to show the performance of our methodology. 

The per-instance accuracy is the most common metric used to assess the performance of the classification. By using accuracy, we were able to compare our results with state-of-the-art methods. These methods will be discussed in detail in the next chapters. For the classification, we used ModelNet-40 due to a well-established classification benchmark associated with this dataset. Unlike the benchmark, we considered three experimental modes to highlight the advantage of our classification pipeline most effectively. The three modes include (1) training and testing with azimuthal rotations (z/z), (2) training and testing with arbitrary rotations  (\textbf{SO(3)}/\textbf{SO(3)}), and (3) training with azimuthal and testing with arbitrary rotations (z/\textbf{SO(3})).

We used the MPEG7 dataset for our retrieval experiments. In literature, the retrieval rate for this dataset is measured by the so-called Bull's Eye score. Every shape in the database is compared to all other shapes, and the number of shapes from the same class among the 40 most similar ones is reported. The Bull's Eye retrieval rate is the ratio of the total number of shapes from the same class to the highest possible number (which is 20 x 1400). Thus, the best possible rate is $1$:

\begin{equation}
    BS = \frac{D_{40}}{P}.
    \label{eq:bullseye_score}
\end{equation}

Where $D_{40}$ is the total sum of correct retrieval instances out of the 40 most similar objects, and $P=20 \times 1400$ is the total possible outcome.

Results of the $BS$ computed on ModelNet40 and classification accuracy on MPEG7 dataset will also be reported and discussed in the following chapters. However, because the benchmarks of the datasets do not use these alternative metrics, it is not possible to show comparative results.

\section{Limitations}

The goal of this research is to study skeleton-based shape description in detail. We aim to explore the properties that make topological skeletons adequate to approach the problem of isometric-invariant shape representation. Despite the long list of classification and retrieval approaches that use a wide range of features inherent to the objects, we are only interested in their shape. Therefore, no photometric or texture information was used in this study. Consequently, the selected datasets only contain information about the geometry of the objects in the form of pre-segmented silhouettes in the 2D case, or triangular meshes without texture in the case of 3D models.

Additionally, in this study, we are interested in exploring isometric invariances and equivariances in shape analysis. For that purpose, we create a classification pipeline based on a deep learning model. Because we do not aim to explore the best deep architecture to classify shapes, we set PointNet++ as our machine learning model. However, we acknowledge that other approaches exist and should be fairly compared with our results.

Although in chapter \ref{ch:introduction}, we discussed a few applications fields where shape analysis has an impact; we do not aim to present any applications of the research problem of this dissertation. This work is limited to assess the performance of the new proposed descriptor in comparison to well-established datasets and benchmarks in the scientific literature.

In this chapter, we defined the employed methodology for this research by describing the two key elements of this work: 1) robust skeletonization and 2) design of classification pipeline based on topological features. In the next chapters, we will further detail both elements and provide a detailed explanation of the experiments conducted and their results.

\newpage

In this chapter, we address the problem of spurious branch removal. Spurious branches in the MAT are associated with noise in the contour. Even a small perturbation can cause a new branch to appear. To address this challenge, we developed a method that produces a consistent skeleton in the presence of several degrees of noise, and show the results of the experiments designed to prove our robust skeletonization. We conducted additional experiments to demonstrate how our method, the CPMA, exhibits equivariance to isometric transformations.

\section{The Cosine-Pruned Medial Axis}

The \textbf{Cosine-Pruned Medial Axis} is defined as a pruned version of the $\mathbf{MAT}$ of a shape $\Omega$. The computation of the CPMA starts with the estimation of the Discrete Cosine Transform ($DCT(\Omega)$). We can reconstruct the original object from the DCT using a truncated number of frequencies $M$.  We repeat this process several times, increasing the value of $i$ each time. By using this method, we assure that each reconstruction is a smooth version of the original object. Each smooth reconstruction is expected to have a skeleton with less spurious branches than the original while still maintaining the skeletal structure.

After computing a set of reconstructions $\mathcal{S} = \left \{ \mathcal{I}^{(i)} \right\}$ for $i=1, 2, ..., M$; we aggregate all of them to create a score function using equation \ref{eq:score_function}, and denote it $\scorefunction$ . Later, the CPMA is the result of thresholding $\scorefunction$ with the parameter $\tau$.

From the above description, it is possible to see how the CPMA can result in a disconnected skeleton. Despite the fact that the CPMA is invariant to contour noise, the connectivity property is necessary to ensure that the topology of the original object is preserved. For this reason, we enforce such connectivity by iteratively connecting the individual parts of the CPMA through a minimum energy path approach. We will refer to this result as the CPMA + connectivity.

In the following sections, we summarize the implementation issues encountered while implementing our methodology. We also offer proof of the isometric equivariance of the CPMA.

\subsection{Implementation details}

In this section, we discuss the algorithms that we used to implement the CPMA and the CPMA + connectivity efficiently. We also discuss their complexity and hyper-parameter selection.

We based our code in python programming language due to its simplicity, the vast number of libraries available, and the popularity in the scientific community for academic projects, particularly in machine learning.

The CPMA only relies on one parameter, $\tau$. The value of $\tau$ is a threshold to determine whether a point of $\scorefunction$ is a skeleton point. The value of $\tau$ was defined empirically to be $\tau=0.5$; however, we conducted an additional experiment to show how sensitive the CPMA is to different values of the threshold. This experiment will be described later in subsection \ref{subsec:hyper_parameter_selection}.

Another important consideration to take into account when computing the CPMA is the number of frequencies employed on the reconstruction of the original object through the DCT. We found that using frequencies greater than $\frac{N}{2}$ does not yield significant improvement for the CPMA. Here, all of the objects are enclosed in square images or cubic volumes with side $N$ in length. 

Finally, we describe the implementation issues of connectivity enforcement. We connect the different pieces of the raw CPMA through the minimum energy path, as stated in chapter \ref{ch:skeleton_shape_analysis}. To do so, we create a lattice graph $\mathcal{G} \in \mathbb{Z}^{n}$. A point $p$ representing a pixel or a voxel, is a node of $\mathcal{G}$, if and only if $p \in \Omega$. The node $p$ shares an edge with every one of its neighbors in the lattice if they are inside $\Omega$. We used an 8-connectivity neighborhood in 2D and a 26-connectivity neighborhood in 3D. 

To determine the minimum energy path between pairs of pixels/voxels with this methodology, we compute the minimum path in the graph using Dijkstra’s algorithm. The weights of each edge are the average of two neighboring values $\mathcal{E}_{\Omega}$, e.g.

\begin{displaymath}
     \textrm{weight}(e_{x, y}) = 0.5(\mathcal{E}(x) + \mathcal{E}(y)).
\end{displaymath}

This method guarantees the connectivity, but it is inefficient because it is based on an iterative computation of the minimum energy path. We sacrifice performance in favor of connectivity. The algorithm for the computation of the CPMA is presented in detail in algorithm \ref{alg:cpma}. Additionally, the connectivity enforcement procedure is explained in algorithm \ref{alg:connect_skeleton_segments}.

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/score_function_1.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/score_function_2.png}
    \end{subfigure}
    
    \caption[Score Function.]{Score Function illustrative example. The images show from left to right the reconstructed object $\Omega$, the score function $F_{\Omega}$ and the real medial axis of $\Omega$. The first row shows the $F_{\Omega}$ computed with reconstructions up to only $M_{1}$ of the first frequencies. The second row shows $F_{\Omega}$ computed with reconstructions up to $M_{2}$ of the first frequencies. $M_{2} > M_{1}$.}
     \label{fig:score_function}
\end{figure}

%- Algorithm

\begin{algorithm}[!ht]

    \SetAlgoLined
    \DontPrintSemicolon
    
    \textbf{Input:}\;
    \hspace{0.15\linewidth} $\mathcal{I}$: N-dimensional binary array representing the object\;
    \hspace{0.15\linewidth} \textbf{M:} number of frequencies of $\mathcal{I}$ to be used in the computation\;
    \textbf{Output:}\;
    \hspace{0.15\linewidth} \textbf{CPMA:} Cosine-Pruned Medial Axis\;
    
    \vspace{0.02\linewidth}
    
    $\tau \gets  0.5$\;
    $\mathfrak{F} \gets DCT(\mathcal{I})$\;
    
    $i \gets 1$\;
    \While{$i < M$}{
        $\hat{\mathcal{I}}^{(i)} = IDCT(\mathfrak{F}, i)$ \tcp*{Reconstruction of $\mathcal{I}$ using only the first $i$ frequencies}
        $\scorefunction = \scorefunction + \mathbf{MAT}(\hat{\mathcal{I}}^{(i)})$\;
        $i \gets i + 1$\;
    }
    $\scorefunction \gets \scorefunction / M$ \tcp*{The final $\scorefunction$ is the average of all reconstructions}\;
    CPMA = $\scorefunction > \tau$\;
    \Return CPMA\;
    
    \caption{Cosine-Pruned Medial Axis (CPMA)}
    \label{alg:cpma}
\end{algorithm}

\begin{algorithm}[!ht]
    \SetAlgoLined
    \DontPrintSemicolon
    
    \textbf{Input:}\;
    \hspace{0.15\linewidth} \textbf{CPMA:} Cosine-Pruned Medial Axis\; representing the object\;
    \hspace{0.15\linewidth} $\scorefunction$ Score function\;
    \textbf{Output:}\;
    \hspace{0.15\linewidth} \textbf{C-CPMA:} Connected Cosine-Pruned Medial Axis\;
    
    \vspace{0.02\linewidth}
    
    C-CPMA $\gets$ \textbf{copy}(CPMA)\;
    skeleton-parts $\gets$ \textbf{compute-skleton-parts}(CPMA)
    
    max-iter $\gets 200$\;
    it $\gets 0$\;
    \While {it $<$ max-iter \textbf{and} $|\textrm{skeleton-parts}| > 1$}{
    
        graph-i $\gets$ skeleton-parts[0]\;
        graph-f $\gets$ skeleton-parts[1]\;
        \tcp{Finds the minimum path inside the object for two pieces of the skeleton }
        min-path $\gets$ \textbf{find-min-path}(graph-i, graph-f, $\scorefunction$)\;
        
        C-CPMA[path] $\gets$ True\;
        
        skeleton-parts $\gets$ \textbf{compute-skeleton-parts}(C-CPMA)\;
        it $\gets$ it + $1$\;
    }
    \Return C-CPMA\;
    
    \caption{Connect skeleton segments}
    \label{alg:connect_skeleton_segments}
\end{algorithm}

\subsection{Isometric Equivariance of the CPMA}

Because distance transform-based skeletons depend only on the shape $\Omega$, and not on the position or size in the embedding space, skeletons should be equivariant under isometric transformations $R$ of $\Omega$, i.e., $\mathbf{MAT}(R(\Omega)) = R(\mathbf{MAT}(\Omega))$. To prove this equivariance, we start from the definition of the MAT

\begin{displaymath}
     \mathbf{MAT}(\Omega) = \left\{ (X, r) \mid X \in \Omega \land B_{r}(X) \not \nsubseteq B_{r ^{\prime}}(X^{\prime}), \forall r^{\prime} > r, X^{\prime} \in \Omega  \right \},
\end{displaymath}

where $B_{r}(X)$ is closed ball centered in $X$ with radius $r$. If we apply an isometric transformation $R$ on $\mathbf{MAT}(\Omega)$ we obtain

\begin{displaymath}
     R(\mathbf{MAT}(\Omega)) = \left\{ (R(X), r) \mid X \in \Omega \land B_{r}(X) \not \nsubseteq B_{r ^{\prime}}(X ^{\prime}), \forall r^{\prime} > r, X^{\prime} \in \Omega  \right \}.
\end{displaymath}

To compute $R(\mathbf{MAT}(\Omega))$ we only need to transform the elements of the result set. As the transformation does not have any effect on the radius, it is easy to verify that $X \in \Omega$ if and only if $R(X) \in R(\Omega)$. As a consequence, $B_{r}(R(X)) \not \nsubseteq B_{r ^{\prime}}(R(X^{\prime})), \forall r^{\prime} > r, R(X^{\prime}) \in R(\Omega)$. Let us now define $Y = R(X)$.  We then have that

\small{
\begin{align*}
    R(\mathbf{MAT}(\Omega)) =& \left\{ (R(X), r) \;\mid\; X \in \Omega \;\land\; [B_{r}(X) \not \nsubseteq B_{r ^{\prime}}(X^{\prime}), \forall r^{\prime} > r, X^{\prime} \in \Omega]  \right \} \\
     =& \left\{ (R(X), r) \;\mid\; R(X) \in R(\Omega) \;\land\; [B_{r}(R(X)) \not \nsubseteq B_{r ^{\prime}}(R(X^{\prime})), \forall r^{\prime} > r, R(X^{\prime}) \in R(\Omega)]  \right \} \\
     =& \left\{ Y, r) \;\mid\; Y \in R(\Omega) \;\land\; [B_{r}(Y) \not \nsubseteq B_{r ^{\prime}}(Y^{\prime}), \forall r^{\prime} > r, Y^{\prime} \in R(\Omega)]  \right \} \\
     =& \;\mathbf{MAT}(R(\Omega))
\end{align*}
}

Our method, the CPMA, depends entirely on $\scorefunction$, which also holds the isometric equivariant property. In fact, by using the above result, and recalling that $R$ is a linear transformation, we can demonstrate that

\begin{displaymath}
     R(\scorefunction) = R\left(\frac{1}{M}\sum_{i=1}^{M} \mathbf{MAT}( \hat{\mathcal{I}}^{(i)})\right) = \frac{1}{M}\sum_{i=1}^{M} R\left(\mathbf{MAT}( \hat{\mathcal{I}}^{(i)})\right) = \frac{1}{M}\sum_{i=1}^{M} \mathbf{MAT}\left( R(\hat{\mathcal{I}}^{(i)})\right)  = \mathcal{F}_{R(\Omega)},
\end{displaymath}

hence proving that the CPMA is equivariant to isometries.

Analytic methods typically satisfy this property because all computations are done in high-precision, continuous vector space. In contrast, discrete methods cannot be fully equivariant because samples of both $\Omega$ and MAT($\Omega$) are constrained to the fixed voxel grid. Additionally, the equivariance of the MAT is also affected by the use of the discrete cosine transform. In a continuous domain, it is easy to demonstrate that the cosine transform, as well as the Fourier Transform, have exact isometric equivariance; however, in a discrete domain, this equivariance is only an approximation, $R(\scorefunction) \approx \mathcal{F}_{R(\Omega)}$. 

\section{Experiments and Results}

\subsection{Comparative Studies}

We chose a set of seven of the most relevant methods in the scientific literature to compare with CPMA skeletonization results. These methods were selected based on a careful review of the state-of-the-art on skeletonization. These methods were also chosen to illustrate the variety of approaches authors employ to pruning the medial axis. The first method we used in our comparative study is the MAT itself without any pruning. The MAT is computed by first calculating the distance transform of the image. The MAT then lies along the singularities (i.e., creases or curvature discontinuities) in the distance transform.

We chose the most representative pruning methods of the state-of-the-art. In general, pruning methods use parameters derived from the distance transform and the projection of a point $x$ in the MAT to the nearest background point of the object, $P_{x}$. However, other factors, such as contour curvature, are also used. Table \ref{tab:skeletonization_comparative_study} summarizes all of the studies employed in our comparative study for 2D. For each method, we used values for the parameters that are the most common through other comparative studies in previous works. In the following sections, we will also show how the CPMA parameter $\tau$ is stable across different objects and even different datasets.

\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{p{0.25\linewidth}cp{0.25\linewidth}p{0.25\linewidth}}
        \hline
        \textbf{{Method}} & \textbf{{Abbreviation}} & \textbf{{Authors}} & \textbf{Parameter} \\
        \hline
        \multicolumn{4}{c}{2D methods} \\
        \hline
        Medial Axis Transform & MAT & \cite{Blum1967} & N/A \\
        Zhang-Suen Algorithm & Thinning & \cite{Zhang1984} & N/A \\
        Gamma Integer Medial Axis & GIMA & \cite{Hesselink2008} & $\mathbf{\gamma}$: minimum distance between $\mathcal{P}_{x}$ and $\mathcal{P}_{y}$, $y \in N_{x}$. \\
        Bisector Euclidean Medial Axis & BEMA & \cite{Couprie2007} & $\mathbf{\theta}$: angle formed by the point $x$ and the two projections $\mathcal{P}_{x}$ and $\mathcal{P}_{y}$, $y \in N_{x}$.\\
        Scale Axis Transform & SAT & \cite{Giesen2009} & $\mathbf{s}$: scale factor to resize $\textbf{MAT}(\Omega)$.  \\
        Scale Filtered Euclidean Medial Axis &  SFEMA & \cite{Postolski2014} & $\mathbf{s}$: scale factor for individual balls in the $\textbf{MAT}(\Omega)$. \\
        Poisson Skeleton & Poisson skel. & \cite{Aubert2014} & $\mathbf{w}$: window size to find the local maximum of contour curvature.\\
        \hline
        \multicolumn{4}{c}{3D methods} \\
        \hline
        Zhang-Suen Algorithm & Thininng & \citep{Zhang1984} & N/A \\
        Tree-structure skeleton extraction & TEASAR & \citep{Sato2000} & N/A \\
        \hline
    \end{tabular}
    \caption[Pruning methods employed for the comparative study in 2D]{Pruning methods employed for the comparative study in 2D. The table shows author, name, and parameter description for each method. The point $x \in \textbf{MAT}$ is element of the MAT that might be pruned. $P_{x}$ refers to the closest boundary point of $x$, while $N_{x}$ accounts for the neighborhood around it.}
    \label{tab:skeletonization_comparative_study}
\end{table}

\subsection{Stability Under Noisy Boundary}

Medial axes are notoriously sensitive to border noise. Because we argue that the CPMA cope reasonably well with shape deformation, it is useful to test how it performs in practice. We, therefore, compared the stability of the CPMA with the other approaches in table \ref{tab:skeletonization_comparative_study}, with respect to contour noise. We based our 2D experiments on Kimia216 and the Animal Dataset for 2D. Additionally, we used a set of three-dimensional objects from the Groningen Benchmark for 3D.

To introduce noise to the boundary of an object, we use two methods: one for 2D and one for 3D. In the 2D case, we deform the random points in the contour of the object in a direction orthogonal to them. Let $\gamma(i) = \left [ x(i), y(i) \right ]$ be the coordinates of the point $i$ in the contour, and let $N_{i}$ be all the neighbor points of $\gamma(i)$ in the contour. The deformation process is applied to a random number of points in the contour such that 

\begin{equation}
    \skew{-.5}\hat \gamma (j) = \gamma(j) + \delta . \lambda . \vec{v} \textrm{ , } \forall j \in N_{i} 
\end{equation}

Where $\vec{v} = [ \begin{array}{cc} -y^{\prime}(i) & x^{\prime}(i) \end{array} ]^{T}$ is a vector normal to the curve in $i$, $\delta$ randomly takes the values $1$ or $-1$, and $\lambda$ is a random variable such that $\lambda \sim \mathcal{N}(i, \sigma)$. Our noise model produces protrusions around random points in the contour chosen with uniform distribution and probability of be deformed of $p=0.005$.

In the 3D case, we propose a simple mechanism to deform the object using a process derived from the Eden’s (accretion) process. The Eden’s process is an iterative random cellular automaton that, in its simplest form, attributes an equal probability to all the outer border points to be set to 1 at each step. That is, at each step, a neighbor of the object is chosen randomly and added to the shape. As a result, the object’s homotopy type remains unchanged at each step. For both 2D and 3D, we denote by $E(\Omega, k)$ the result of applying $k$ steps of the noise model to the shape $\Omega$. %Figure \ref{fig:noise_model_examples} show examples of objects from Kimia216 and Animal2000 datasets, for several levels of noise. 

For our noise sensitivity experiments, we apply $20$ times $E(\Omega, k)$ to every object of every dataset, and then compute its MAT using every method in table \ref{tab:skeletonization_comparative_study} with different parameters. Later, each $\mathbf{MAT}(E(\Omega, k))$ is compared with $\mathbf{MAT}(\Omega)$ using both the Hausdorff distance and Dubuisson-Jain dissimilarity. Finally, we report the per method average of each metric over all the elements of each dataset.

%\begin{figure}[!ht]
%    \centering
%    \includegraphics[width=0.8\linewidth]{example-image-a}
%    
%    \caption[Noise model applies to elements of each dataset]{Noise model applies to elements of each datasets (rows). From top to bottom: Kimia216, Animal2000 and Groningen Benchmark. The images illustrate  the noise deformation process, after 0 (original image), 10, and 15 steps. TODO}
%     \label{fig:noise_model_examples}
%\end{figure}

%- Talk about the results. For Kimia

We first test our skeletonization method on the Kimia216 dataset. We used all methods from table \ref{tab:skeletonization_comparative_study} with different input parameters, and compared them to the CPMA and the CPMA with connectivity enforcement. The parameters for each method were chosen empirically as the most commonly employed parameters in literature. The results for all methods are shown in table \ref{tab:noise_sensitivity_results_kimia}. This table shows how our methods are competitive against state-of-the-art skeletonization methods such as the GIMA and SFEMA, and perform better than methods such as Poisson Skeletons, SAT, skeletonization by thinning, and the MAT itself. Figure \ref{fig:noise_results_kimia} shows both Hausdorff distance and Dubuisson-Jain dissimilarity against noise level. The figure only displays the curves with the parameters that yielded the best performance for every method in the comparative study. Note that for most methods, the results are approximately the same for low levels of noise; however, the curves (and the values in the table) start diverging when the noise level increases, revealing the real noise invariant properties.  In the figure, it is also possible to see how the CPMA and the CPMA+connnect are among the three best results when the dissimilarity metric is used, only surpassed by the GIMA. Although the results are not as good compared to methods with the Hausdorff distance, it is possible to see how our methods still fall among the top five results. 

\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{l|cccc|cccc}
        \hline
        \textbf{{Method}} & \multicolumn{4}{c}{\textbf{{Hausdorff}}} & \multicolumn{4}{c}{\textbf{{Dissimilarity}}} \\
          & 5 & 10 & 15 & 20  & 5 & 10 & 15 & 20 \\
        \hline
        MAT  & 8.13 & 8.50 & 8.43 & 9.41  & 1.95 & 2.67 & 3.01 & 3.27 \\
        Thinning  & 4.68 & 5.85 & 6.88 & 8.15  & 2.18 & 3.26 & 3.94 & 4.45 \\
        GIMA (r=5)  & 5.46 & 6.50 & 7.37 & 8.84  & 0.87 & 1.31 & 1.60 & 1.88 \\
        GIMA (r=10)  & 5.40 & 7.12 & 8.35 & 9.18  & 0.68 & 1.07 & 1.35 & 1.58 \\
        \textbf{GIMA (r=20)}  & \textbf{4.49} & \textbf{5.76} & \textbf{6.39} & \textbf{7.30}  & \textbf{1.00} & \textbf{1.30} & \textbf{1.05} & \textbf{1.35} \\
        BEMA (theta=90)  & 5.22 & 6.55 & 7.11 & 8.30  & 0.99 & 1.60 & 2.07 & 2.53 \\
        BEMA (theta=120)  & 5.05 & 6.56 & 7.60 & 8.74  & 0.70 & 1.37 & 1.94 & 2.52 \\
        BEMA (theta=150)  & 6.68 & 7.69 & 7.89 & 9.40  & 0.99 & 1.80 & 2.50 & 3.37 \\
        SAT (s=1.1)  & 8.68 & 8.73 & 8.76 & 9.64  & 3.09 & 4.37 & 5.08 & 5.57 \\
        SAT (s=1.2)  & 9.61 & 10.05 & 9.79 & 10.20  & 2.50 & 3.22 & 3.89 & 4.47 \\
         SFEMA (s=1.1)  & 4.15 & 5.35 & 6.18 & 7.53  & 0.84 & 1.37 & 1.92 & 2.50 \\
         SFEMA (s=1.2)  & 3.64 & 5.13 & 6.15 & 7.64  & 0.68 & 1.11 & 1.53 & 1.99 \\
        Poisson skel. (w=0.05)  & 11.43 & 11.16 & 11.26 & 12.73  & 2.46 & 3.05 & 3.27 & 3.53 \\
        Poisson skel. (w=0.10)  & 15.60 & 15.48 & 16.07 & 17.35  & 3.62 & 4.07 & 4.19 & 4.56 \\
        \textbf{Poisson skel. (w=0.20)}  & \textbf{17.71} & \textbf{18.02} & \textbf{19.54} & \textbf{21.35}  & \textbf{5.00} & \textbf{5.38} & \textbf{5.63} & \textbf{6.20} \\
        \hline
        CPMA  & 5.55 & 7.28 & 8.07 & 9.66  & 0.71 & 1.08 & 1.39 & 1.71 \\
        CPMA + Connect.  & 5.19 & 6.68 & 7.66 & 9.12  & 0.80 & 1.20 & 1.58 & 1.94 \\
        \hline
    \end{tabular}
    \caption[Noise sensitivity results on Kimia216]{Noise sensitivity results on Kimia216. The table shows the average Hausdorff distance and Dubuisson-Jain dissimilarity for different noise levels (5-20) over each element of the dataset. The best and worst method are highlighted to facilitate the comparison with the CPMA.}
    \label{tab:noise_sensitivity_results_kimia}
\end{table}

%NOTE: Hausdorff images are cropped to 455 in width
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.41\linewidth}
        \includegraphics[width=\linewidth]{images/kimia_best_Hausdorff_distance_noisy.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.58\linewidth}
        \includegraphics[width=\linewidth]{images/kimia_best_Dissimilarity_measure_noisy.png}
    \end{subfigure}
    
    \caption[Noise sensitivity results on Kimia216 dataset]{Noise sensitivity results on Kimia216 dataset. The figure shows the Hausdorff distance (left) and the Dubuisson-Jain dissimilarity (right) for all the methods in table \ref{tab:noise_sensitivity_results_kimia}. Only the best parametrization of each method is depicted for better interpretation.}
    \label{fig:noise_results_kimia}
\end{figure}

The Animal2000 dataset contains nearly ten times more shapes than Kimia216. The Animal2000 dataset consists of 2000 images of different animals in a wide variety of poses. This implies more variation between shapes, and therefore a more challenging setting. Table \ref{tab:noise_sensitivity_results_animal} shows similar results compared to Kimia216, confirming that the noise invariant properties of the CPMA still hold in a more robust dataset. The GIMA is still the best method measured with the Dubuisson-Jain dissimilarity, and it is followed closely by both the CPMA and the CPMA with connectivity enforcement. Results of using the Hausdorff distance as a metric show that the CPMA is close to methods such as BEMA and SFEMA; however, the results are not as good as when using the dissimilarity. Figure \ref{fig:noise_results_animal} depicts the best performance for every method in comparison to ours. Our results suggest that the CPMA noise invariant properties generalize across different datasets because of the complexity of Animal2000 regarding the number of shapes and the diversity of those shapes. Note that that results in figure \ref{fig:noise_results_animal} appear to be smoother than those in the previously discussed figure \ref{fig:noise_results_kimia} on Kimia216. For further inspection, we include figures of all methods and all parameters in appendix \ref{apx:noise_sensitivity}.

\begin{table}[!ht]
    \centering
    \small
    
    \begin{tabular}{l|cccc|cccc}
        \hline
        \textbf{{Method}} & \multicolumn{4}{c}{\textbf{{Hausdorff}}} & \multicolumn{4}{c}{\textbf{{Dissimilarity}}} \\
          & 5 & 10 & 15 & 20  & 5 & 10 & 15 & 20 \\
        \hline
        MAT  & 7.47 & 10.39 & 12.47 & 14.64  & 3.56 & 4.50 & 5.00 & 5.29 \\
        Thinning  & 7.51 & 10.79 & 12.94 & 15.03  & 2.30 & 3.71 & 4.52 & 4.99 \\
        GIMA (r=5)  & 7.96 & 11.00 & 13.23 & 15.27  & 1.24 & 1.88 & 2.35 & 2.68 \\
        GIMA (r=10)  & 6.78 & 8.56 & 10.21 & 11.54  & 0.89 & 1.29 & 1.62 & 1.89 \\
        \textbf{GIMA (r=20)}  & \textbf{5.02} & \textbf{6.86} & \textbf{8.29} & \textbf{9.77}  & \textbf{0.85} & \textbf{1.16} & \textbf{1.52} & \textbf{1.89} \\
        BEMA (theta=90)  & 7.84 & 10.61 & 12.76 & 14.78  & 1.45 & 2.37 & 3.06 & 3.57 \\
        BEMA (theta=120)  & 7.86 & 11.76 & 13.93 & 15.74  & 1.22 & 2.25 & 3.04 & 3.69 \\
        BEMA (theta=150)  & 8.88 & 12.38 & 14.39 & 16.51  & 1.68 & 3.00 & 3.95 & 4.72 \\
        SAT (s=1.1)  & 9.44 & 11.80 & 13.47 & 15.21  & 2.80 & 4.13 & 5.02 & 5.49 \\
        SAT (s=1.2)  & 11.28 & 13.57 & 15.21 & 16.40  & 2.13 & 3.13 & 3.85 & 4.55 \\
         SFEMA (s=1.1)  & 7.44 & 11.00 & 13.30 & 15.35  & 1.33 & 2.27 & 3.03 & 3.69 \\
         SFEMA (s=1.2)  & 7.64 & 11.43 & 13.83 & 15.90  & 1.26 & 2.13 & 2.78 & 3.36 \\
        Poisson skel. (w=0.05)  & 11.94 & 13.68 & 15.35 & 17.03  & 3.08 & 3.63 & 4.01 & 4.20 \\
        Poisson skel. (w=0.10)  & 14.55 & 17.11 & 18.64 & 20.10  & 3.55 & 4.08 & 4.68 & 4.94 \\
        \textbf{Poisson skel. (w=0.20)}  & \textbf{17.37} & \textbf{20.35} & \textbf{21.67} & \textbf{23.69}  & \textbf{3.94} & \textbf{4.69} & \textbf{5.33} & \textbf{5.73} \\
        \hline
        CPMA  & 9.20 & 12.88 & 14.96 & 17.22  & 1.18 & 1.96 & 2.55 & 3.09 \\
        CPMA + Connect.  & 8.67 & 12.39 & 14.45 & 16.88  & 1.17 & 1.96 & 2.58 & 3.13 \\
        \hline
    \end{tabular}
    
    \caption[Noise sensitivity results on Animal2000]{Noise sensitivity results on Animal2000. The table shows the average Hausdorff distance and Dubuisson-Jain dissimilarity for different noise levels (5-20) over each element of the dataset. The best and worst methods are highlighted to facilitate the comparison to the CPMA.}
    \label{tab:noise_sensitivity_results_animal}
\end{table}

%NOTE: Hausdorff images are cropped to 455 in width
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.41\linewidth}
        \includegraphics[width=\linewidth]{images/animal_best_Hausdorff_distance_noisy.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.58\linewidth}
        \includegraphics[width=\linewidth]{images/animal_best_Dissimilarity_measure_noisy.png}
    \end{subfigure}
    
    \caption[Noise sensitivity results on Animal2000 dataset]{Noise sensitivity results on Animal2000 dataset. The figure shows the Hausdorff distance (left) and the Dubuisson-Jain dissimilarity (right) for all the methods in table \ref{tab:noise_sensitivity_results_animal}. Only the best parametrization of each method is depicted for better interpretation.}
    \label{fig:noise_results_animal}
\end{figure}

For our 3D experiments, we picked 14 objects from the Groningen benchmark, reflecting the most common shapes used in the literature. Each object was voxelized to a binary voxel grid with resolution $150 \times 150 \times 150$. This resolution offers sufficient details as well as a sufficiently low computational cost. In contrast to the 2D case, we apply $E(\Omega, k)$ only $10$ times to the 3D object. We did this for two reasons: 1) to reduce computational complexity, and 2) because in 3D with the chosen resolution, noise tends to be more extreme. The results on the Groningen dataset are shown in table \ref{tab:noise_sensitivity_results_groningen} and figure \ref{fig:noise_results_gronigen}. We can observe that both the CPMA and CPMA+connectivity achieved the best results among other methods when compared with the dissimilarity measure. These results are evidence that our methodology has noise-invariance properties, and it is stable in the presence of contour of surface deformation. However, the results show unusual patterns when compared with the Hausdorff distance. In fact, for some methods, the metric decreases when the noise level increases. We attribute this behavior to the outlier sensibility of the Hausdorff distance.

\begin{table}[!ht]
    \centering
    \small
    
    \begin{tabular}{l|ccccc|ccccc}
        \hline
        \textbf{{Method}} & \multicolumn{5}{c}{\textbf{{Hausdorff}}} & \multicolumn{4}{c}{\textbf{{Dissimilarity}}} \\
          & 2 & 4 & 6 & 8 & 10  & 2 & 4 & 6 & 8 & 10 \\
        \hline
        3D thinning  & \textbf{4.20} & \textbf{3.61} & \textbf{3.25} & \textbf{3.03} & \textbf{2.90}  & 6.30 & 7.80 & 8.58 & 9.07 & 9.41 \\
        TEASAR  & 7.76 & 7.36 & 6.39 & 6.24 & 5.92  & 1.09 & 1.55 & 1.98 & 2.44 & 2.80 \\
        \hline
        CPMA  & 11.66 & 14.10 & 11.83 & 15.52 & 12.46  & 0.91 & 1.02 & 0.97 & 1.44 & 1.27 \\
        CPMA + Connect.  & 3.99 & 4.54 & 11.25 & 13.95 & 12.06  & \textbf{0.40} & \textbf{0.43} &\textbf{1.43} & \textbf{1.81} & \textbf{1.51} \\
        \hline
    \end{tabular}
    
    \caption[Noise sensitivity results on Groningen benchmark]{Noise sensitivity results on Groningen benchmark. The table shows the average Hausdorff distance and Dubuisson-Jain dissimilarity for different noise levels (5-20) over each element of the dataset. The best result is highlighted in bold font for comparison.}
    \label{tab:noise_sensitivity_results_groningen}
\end{table}

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.41\linewidth}
        \includegraphics[width=\linewidth]{images/groningen_Hausdorff_distance_noisy.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.58\linewidth}
        \includegraphics[width=\linewidth]{images/groningen_Dissimilarity_measure_noisy.png}
    \end{subfigure}
    
    \caption[Noise sensitivity results on Groningen Benchmark dataset]{Noise sensitivity results on Groningen Benchmark dataset. The figure shows the Hausdorff distance (left) and the Dubuisson-Jain dissimilarity (right) for all the methods in table \ref{tab:noise_sensitivity_results_groningen}.}
    \label{fig:noise_results_gronigen}
\end{figure}

We complete the noise stability analysis showing some examples of the MAT computed with our methodology, in comparison with the MAT computed using other methods in the comparative study. Figure \ref{fig:mat_examples_noise} shows such comparisons for all the datasets above mentioned datasets.

\begin{figure}
    \centering
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/Kimia_2_cropped.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/Kimia_1_cropped.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/Animal_9_cropped.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/Animal_3_cropped.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/Dragon_results.png}
    \end{subfigure}
    
    \begin{subfigure}[b]{\linewidth}
        \includegraphics[width=\linewidth]{images/Frog_results.png}
    \end{subfigure}
    
    \caption[Skeletonization results]{Skeletonization results. The images show the MAT and the results of four different pruning methods. Rows one and two are objects from Kimia216, rows three and four are from Animal2000, and rows five and six from the Groningen benchmark. Notice how the CPMA and the CPMA + connectivity produces skeletons with less spurious branches while preserving the topology.}
    \label{fig:mat_examples_noise}
\end{figure}

\subsection{Sensitivity to Rotations}

In the continuous framework, it is well known that the medial axis is a rotation equivariant shape representation. More precisely, if we denote by $R$ the rotation matrix around the origin; the rotation equivariance property states that $\mathbf{MAT}(R(\Omega)) \approx R(\mathbf{MAT}(\Omega))$. Regardless of the shape $\Omega$ and the rotation $R$.

Nevertheless, we can experimentally measure the dissimilarity between $\mathbf{MAT}(R(\Omega))$ and $R(\mathbf{MAT}(\Omega))$ for different instances, and different definitions of the medial axis transform. The lower this dissimilarity, the more stable the method is under rotation. We conducted experiments on Kimia216, Animal2000, and the Groningen Benchmark by inducing a set of controlled rotations on each element of every dataset. Later, we computed the Hausdorff distance and the Dubuisson-Jain dissimilarity between $\mathbf{MAT}(R(\Omega))$ and $R(\mathbf{MAT}(\Omega))$ for rotation angles varying from $0$ to $90$ degrees by 3 degrees steps in 2D. In the 3D case, we varied the experiments for computational efficiency. We induced azimuthal rotations (around z-axis) and elevation rotations (around y-axis) up to $90$ degrees, but at intervals of $18$ degrees.

The rotation sensitivity analysis on the Kimia216 dataset is summarized in table \ref{tab:rotation_sensitivity_results_kimia} and figure \ref{fig:hausdorff_dissimilarity_rotation_results_kimia}. The results show that the CPMA and the CPMA with connectivity enforcement curves lie near the average of the rest of the methods achieving state-of-the-art performance and even surpassing some of them. Notice that when using the dissimilarity metric, both CPMA, the GIMA, the SFEMA, and the BEMA form a subgroup that performs significantly better compared to the others. Moreover, the performance of these methods oscillates around a value of dissimilarity of around $1$ pixel on average. The intuition for this result is that regardless of the rotation, skeletons computed with these methods vary only at one pixel on average. Consequently, we can claim that they exhibit rotation equivariance.

\begin{table}[!ht]
    \centering
    \small
    \begin{tabular}{l|ccc|ccc}
        \hline
        \textbf{{Method}} & \multicolumn{3}{c}{\textbf{{Hausdorff}}} & \multicolumn{3}{c}{\textbf{{Dissimilarity}}} \\
          & 30º & 60º & 90º  & 30º & 60º & 90º \\
        \hline
        MAT  & 8.18 & 8.17 & 2.17  & 2.67 & 2.64 & 0.75 \\
        Thinning  & 7.72 & 7.58 & 8.92  & 2.87 & 2.99 & 1.35 \\
        GIMA (r=5)  & 6.16 & 6.03 & 5.54  & 1.02 & 1.11 & 0.85 \\
        GIMA (r=10)  & 5.54 & 6.25 & 5.04  & 0.83 & 1.02 & 0.72 \\
        GIMA (r=20)  & 3.62 & 3.93 & 3.12  & 1.51 & 0.78 & 1.30 \\
        BEMA (theta=90)  & 12.35 & 12.76 & 11.72  & 1.31 & 1.60 & 1.06 \\
        BEMA (theta=120)  & 6.24 & 8.44 & 9.57  & 0.81 & 1.00 & 1.00 \\
        BEMA (theta=150)  & 9.14 & 10.09 & 10.27  & 1.11 & 1.35 & 1.36 \\
        SAT (s=1.1)  & 10.84 & 11.93 & 3.96  & 3.22 & 3.34 & 0.97 \\
        SAT (s=1.2)  & 11.44 & 12.40 & 4.45  & 2.64 & 2.87 & 0.97 \\
        SFEMA (s=1.1)  & 3.86 & 3.98 & 2.52  & 0.92 & 1.01 & 0.83 \\
        \textbf{SFEMA (s=1.2)}  & \textbf{3.68} & \textbf{3.66} & \textbf{2.08}  & \textbf{0.82} & \textbf{0.88} & \textbf{0.80} \\
        Poisson skel. (w=0.05)  & 12.83 & 13.32 & 8.93  & 3.21 & 3.28 & 1.30 \\
        Poisson skel. (w=0.10)  & 16.36 & 17.03 & 10.17  & 4.24 & 4.30 & 1.78 \\
        \textbf{Poisson skel. (w=0.20)}  & \textbf{18.94} & \textbf{19.90} & \textbf{9.65}  & \textbf{5.61} & \textbf{5.66} & \textbf{2.69} \\
        \hline
        CPMA  & 8.63 & 8.65 & 2.42  & 1.18 & 1.33 & 0.70 \\
        CPMA + Connect.  & 8.51 & 8.36 & 2.72  & 1.22 & 1.39 & 0.75 \\
        \hline
    \end{tabular}
    \caption[Rotation equivariance results on Kimia216]{Rotation equivariance results on Kimia216. The table shows the average Hausdorff distance and Dubuisson-Jain dissimilarity for different rotations of each element in the dataset. The best and worse method are highlighted to facilitate the comparison with the CPMA.}
    \label{tab:rotation_sensitivity_results_kimia}
\end{table}

%NOTE: Hausdorff images are cropped to 455 in width
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.41\linewidth}
        \includegraphics[width=\linewidth]{images/kimia_best_Hausdorff_distance_rot.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.58\linewidth}
        \includegraphics[width=\linewidth]{images/kimia_best_Dissimilarity_measure_rot.png}
    \end{subfigure}
    
    \caption[Rotation equivariance results on Kimia216 dataset]{Rotation equivariance results on Kimia216 dataset. The top row shows the Hausdorff distance and Dubuisson-Jain dissimilarity for all the methods in table \ref{tab:rotation_sensitivity_results_kimia}. The bottom row shows only the best 5 results for clarification.}
    \label{fig:hausdorff_dissimilarity_rotation_results_kimia}
\end{figure}

We applied the same analysis to the Animal2000 dataset achieving similar results. In this case, the CPMA and the CPMA+connectivity ranked third and fourth, respectively, among all methods when we used the dissimilarity metric. The results for all methods and parameters are presented in table \ref{tab:rotation_sensitivity_results_animal}. As before, we also present a summary with the best parametrization for each method in figure \ref{fig:rotation_results_animal} to facilitate the interpretation. Notice that due to the larger number of objects in the Animal2000 dataset, the curves for every method appear to be smoother, highlighting stability across different rotation angles and shapes.

\begin{table}[!ht]
    \centering
    \small
    
    \begin{tabular}{l|ccc|ccc}
        \hline
        \textbf{{Method}} & \multicolumn{3}{c}{\textbf{{Hausdorff}}} & \multicolumn{3}{c}{\textbf{{Dissimilarity}}} \\
          & 30º & 60º & 90º  & 30º & 60º & 90º \\
        \hline
        MAT  & 5.08 & 5.17 & 2.38  & 3.67 & 3.64 & 0.77 \\
        Thinning  & 5.85 & 6.11 & 4.35  & 1.71 & 1.86 & 0.94 \\
        GIMA (r=5)  & 5.58 & 5.54 & 5.62  & 0.96 & 1.08 & 0.83 \\
        GIMA (r=10)  & 5.42 & 5.50 & 4.29  & 0.78 & 0.88 & 0.74 \\
        \textbf{GIMA (r=20)}  & \textbf{3.17} & \textbf{3.84} & \textbf{3.02}  & \textbf{0.68} & \textbf{0.81} & \textbf{0.66} \\
        BEMA (theta=90)  & 11.12 & 11.92 & 9.80  & 1.10 & 1.35 & 0.89 \\
        BEMA (theta=120)  & 5.45 & 6.10 & 6.80  & 0.77 & 0.90 & 0.86 \\
        BEMA (theta=150)  & 7.60 & 8.88 & 9.91  & 1.13 & 1.36 & 1.40 \\
        SAT (s=1.1)  & 7.41 & 7.27 & 3.90  & 2.10 & 2.16 & 0.86 \\
        SAT (s=1.2)  & 9.82 & 9.62 & 4.85  & 1.77 & 1.90 & 0.95 \\
         SFEMA (s=1.1)  & 3.52 & 3.54 & 2.45  & 0.84 & 0.93 & 0.83 \\
         SFEMA (s=1.2)  & 3.54 & 3.63 & 2.26  & 0.77 & 0.87 & 0.82 \\
        Poisson skel. (w=0.05)  & 12.88 & 12.72 & 10.18  & 3.33 & 3.40 & 1.54 \\
        Poisson skel. (w=0.10)  & 15.02 & 15.41 & 10.58  & 3.67 & 3.89 & 1.89 \\
        \textbf{Poisson skel. (w=0.20)}  & \textbf{16.83} & \textbf{17.20} & \textbf{8.67}  & \textbf{4.07} & \textbf{4.33} & \textbf{1.85} \\
        \hline
        CPMA  & 6.62 & 6.14 & 2.64  & 0.96 & 1.06 & 0.77 \\
        CPMA + Connect.  & 6.19 & 5.77 & 3.30  & 0.98 & 1.05 & 0.86 \\
        \hline
    \end{tabular}
    \caption[Rotation equivariance results on Animal2000]{Rotation equivariance results on Animal2000. The table shows the average Hausdorff distance and Dubuisson-Jain dissimilarity for different rotations of each element in the dataset. The best and worse method are highlighted to facilitate the comparison with the CPMA.}
    \label{tab:rotation_sensitivity_results_animal}
\end{table}

%NOTE: Hausdorff images are cropped to 455 in width
\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.41\linewidth}
        \includegraphics[width=\linewidth]{images/animal_best_Hausdorff_distance_rot.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.58\linewidth}
        \includegraphics[width=\linewidth]{images/animal_best_Dissimilarity_measure_rot.png}
    \end{subfigure}
    
    \caption[Rotation equivariance results on Animal2000 dataset]{Rotation equivariance results on Animal2000 dataset. The top row shows the Hausdorff distance and Dubuisson-Jain dissimilarity for all the methods in table \ref{tab:rotation_sensitivity_results_kimia}. The bottom row shows only the best 5 results for clarification.}
    \label{fig:rotation_results_animal}
\end{figure}

Finally, we ran the rotation sensitivity analysis on the 3D datasets, and summarize the results in figure \ref{fig:rotation_results_groningen}. The image shows the four 3D skeletonization methods we used in our study for combinations of azimuthal and elevation angles. This figure illustrates how both the Hausdorff distance and the dissimilarity get higher when the rotation becomes more extreme, except in the case of CPMA + connectivity. We believe this behavior is due to the connectivity enforcement mitigating the gaps in the skeletons, and reducing the metrics.

\begin{figure}[!ht]
    \centering
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{images/groningen_Hausdorff_distance_rot.png}
    \end{subfigure}
    \begin{subfigure}[b]{0.48\linewidth}
        \includegraphics[width=\linewidth]{images/groningen_Dissimilarity_measure_rot.png}
    \end{subfigure}
    
    \caption[Rotation equivariance results on Groningen Benchmark dataset]{Rotation equivariance results on Groningen Benchmark dataset. The top row shows the Hausdorff distance and Dubuisson-Jain dissimilarity for all the methods in table \ref{tab:rotation_sensitivity_results_kimia}. The bottom row shows only the best 5 results for clarification.}
    \label{fig:rotation_results_groningen}
\end{figure}.

\subsection{Hyper-parameter Selection}
\label{subsec:hyper_parameter_selection}

Many medial axis pruning methods depend on hyper-parameters to work correctly. These parameters usually have a physical meaning in the context of the object whose skeleton we sought to estimate. Often, the parameters are distances or angles formed between points inside the object. Some other works also create score function like ours intending to use its values as a filter parameter to remove individual points form the MAT, hoping to reduce the number of spurious branches. However, in most cases, such parameters are subject to factors like resolution or scale. Hence, we conducted another experiment to test the sensitivity of the CPMA to the pruning parameter $\tau$. 

We ran additional experiments for different scale factors of the object. Figure \ref{fig:scale_sensitivity_analysis} shows the average of a reconstruction metric vs the selected value of $\tau$. We compared an object $\Omega$ against its reconstruction $\hat \Omega$ using the Jaccard Index overall images in Kimia216 dataset. High values of $\tau$ deteriorate the reconstruction, while lower values do not prune enough spurious branches. From the figure, we can infer that values around $\tau=0.5$ offer a good trade-off between reconstruction and branch pruning. Moreover, around this value, the standard deviation reaches its minimum value suggesting optimal performance regardless of the object. Because the value of $\tau$ is stable for different scale factors, we conclude that scale does not affect the selection of the threshold.

\begin{figure}[!ht]
    \centering
    \includegraphics[width=0.7\linewidth]{images/cpma_scale_sensitivity_adjust.png}
    
    \caption[Sensitivity Analysis of threshold $\tau$.]{Sensitivity Analysis of threshold $\tau$ to different scales of the input images. The graph shows the average Jaccard index of the reconstructed shape w.r.t the original object for CPMAs computed with different values of $\tau$. Higher values of the threshold lead to less spurious branches. We also show the standard deviation error bands.}
     \label{fig:scale_sensitivity_analysis}
\end{figure}

In the next chapter, we will present experiments in which we use the CPMA + connectivity as input shape representation for our classification and retrieval pipeline. We will derive some features from our skeletonization, and then train a machine learning approach to predict the class of each element.
